Scaling K2. V. Statistical Validation of 60 New Exoplanets From K2 Campaigns 2-18

The NASA K2 mission, salvaged from the hardware failures of the Kepler telescope, has continued Kepler's planet-hunting success. It has revealed nearly 500 transiting planets around the ecliptic plane, many of which are the subject of further study, and over 1000 additional candidates. Here we present the results of an ongoing project to follow-up and statistically validate new K2 planets, in particular to identify promising new targets for further characterization. By analyzing the reconnaissance spectra, high-resolution imaging, centroid variations, and statistical likelihood of the signals of 91 candidates, we validate 60 new planets in 46 systems. These include: a number of planets amenable to transmission spectroscopy (K2-384 f, K2-387 b, K2-390 b, K2-403 b, and K2-398 c), emission spectroscopy (K2-371 b, K2-370 b, and K2-399 b), and both (K2-405 b and K2-406 b); several systems with planets in or close to mean motion resonances (K2-381, K2-398) including a compact, TRAPPIST-1-like system of five small planets orbiting a mid-M dwarf (K2-384); an ultra-short period sub-Saturn in the hot Saturn desert (K2-399 b); and a super-Earth orbiting a moderately bright (V=11.93), metal-poor ([Fe/H]=-0.579+/-0.080) host star (K2-408 b). In total we validate planets around 4 F stars, 26 G stars, 13 K stars, and 3 M dwarfs. In addition, we provide a list of 37 vetted planet candidates that should be prioritized for future follow-up observation in order to be confirmed or validated.

==> Table5-withUncertainties.tex <==
K2-X10 b & $710$ & $8.65\pm5.47$ & $2.2\pm0.14$ & $22.2$ & $1.26$\\%204750116
K2-X26 b & $770$ & $6.34\pm3.66$ & $1.83\pm0.11$ & $18.2$ & $1.14$\\%205111664
K2-X44 b & $450$ & $6.47\pm4.02$ & $1.82\pm0.12$ & $14.6$ & $0.41$\\%206055981
K2-X18 b & $800$ & $2.34\pm1.34$ & $1.06\pm0.07$ & $1.7$ & $0.58$\\%206135682
K2-X18 d & $650$ & $2.49\pm1.31$ & $0.91\pm0.06$ & $1.4$ & $0.35$\\%206135682
K2-X18 c & $500$ & $4.64\pm2.73$ & $1.32\pm0.08$ & $10.9$ & $0.31$\\%206135682
K2-X45 b & $1080$ & $2.2\pm1.3$ & $0.96\pm0.06$ & $2.3$ & $0.82$\\%206146957
EPIC 206317286 c & $570$ & $5.37\pm3.13$ & $1.49\pm0.09$ & $7.6$ & $0.32$\\%206317286
K2-XX4 b & $1420$ & $10.42\pm6.6$ & $5.23\pm0.32$ & $71.1$ & $9.92$\\%210797580
K2-XX1 b & $1000$ & $1497.88\pm6298.5$ & $673.18\pm43.22$ & $8.0$ & $37.84$\\%211399359
K2-X27 b & $870$ & $9.2\pm5.37$ & $3.07\pm0.06$ & $12.6$ & $1.01$\\%211490999
K2-X46 b & $1130$ & $5.15\pm2.85$ & $1.34\pm0.08$ & $13.9$ & $1.02$\\%211539054
K2-X23 b & $1210$ & $3.62\pm1.87$ & $1.72\pm0.03$ & $9.7$ & $0.75$\\%211732116
K2-X23 c & $790$ & $5.71\pm3.48$ & $1.77\pm0.03$ & $10.8$ & $0.58$\\%211732116
K2-X28 b & $1000$ & $5.83\pm3.37$ & $1.42\pm0.09$ & $4.3$ & $0.31$\\%212006318
k2-x47 b & $1240$ & $4.1\pm2.36$ & $1.56\pm0.1$ & $20.6$ & $1.61$\\%212222383
K2-X30 b & $530$ & $3.93\pm2.34$ & $1.22\pm0.08$ & $7.7$ & $0.31$\\%212530118
K2-X25 b & $1130$ & $9.02\pm5.52$ & $4.78\pm0.31$ & $11.6$ & $1.55$\\%212575828
K2-X31 b & $680$ & $5.59\pm3.33$ & $1.92\pm0.12$ & $16.6$ & $1.03$\\%214173069
K2-X32 b & $1110$ & $7.96\pm4.6$ & $2.42\pm0.15$ & $19.4$ & $1.79$\\%214419545
K2-X11 b & $670$ & $1.28\pm0.83$ & $0.5\pm0.03$ & $1.7$ & $0.34$\\%217192839
K2-X11 d & $530$ & $5.04\pm3.01$ & $1.54\pm0.1$ & $14.9$ & $0.57$\\%217192839
K2-X11 c & $440$ & $3.85\pm2.25$ & $0.99\pm0.06$ & $9.7$ & $0.20$\\%217192839
K2-XX9 b & $610$ & $5.15\pm3.23$ & $1.25\pm0.08$ & $10.2$ & $0.37$\\%217977895
K2-X33 b & $1270$ & $3.26\pm1.66$ & $1.63\pm0.1$ & $18.4$ & $1.70$\\%218668602
K2-X21 f & $600$ & $1.28\pm0.83$ & $1.57\pm0.01$ & $6.3$ & $1.44$\\%220221272
K2-X21 d & $480$ & $1.72\pm0.86$ & $1.7\pm0.01$ & $5.1$ & $0.83$\\%220221272
K2-X21 c & $410$ & $2.71\pm1.4$ & $2.3\pm0.01$ & $4.4$ & $0.60$\\%220221272
K2-X21 e & $370$ & $2.39\pm1.36$ & $1.79\pm0.01$ & $4.1$ & $0.35$\\%220221272
K2-X21 b & $330$ & $5.71\pm3.33$ & $3.82\pm0.02$ & $45.6$ & $0.54$\\%220221272
K2-X19 b & $1100$ & $3.2\pm1.79$ & $1.61\pm0.1$ & $7.5$ & $0.66$\\%220459477
k2-x34 b & $1010$ & $6.21\pm3.66$ & $2.16\pm0.03$ & $11.5$ & $0.87$\\%220510874
K2-X20 b & $340$ & $45.46\pm31.68$ & $13.8\pm0.2$ & $23.1$ & $0.83$\\%220696233
K2-XX2 b & $970$ & $13.1\pm8.36$ & $5.07\pm0.32$ & $30.3$ & $3.33$\\%245943455
K2-X17 c & $1050$ & $5.65\pm3.3$ & $2.05\pm0.13$ & $16.4$ & $1.24$\\%245991048
K2-X17 b & $780$ & $5.26\pm2.73$ & $1.41\pm0.09$ & $10.7$ & $0.55$\\%245991048
k2-x37 b & $1310$ & $20.24\pm12.4$ & $10.17\pm0.63$ & $30.3$ & $5.63$\\%245995977
K2-XX8 b & $900$ & $2.49\pm1.71$ & $1.15\pm0.07$ & $3.3$ & $1.06$\\%246074314
K2-XX3 b & $840$ & $4.45\pm2.52$ & $1.28\pm0.08$ & $6.4$ & $0.36$\\%246084398
k2-x35 b & $950$ & $6.34\pm4.06$ & $2.02\pm0.12$ & $15.6$ & $1.16$\\%246429049
k2-x36 b & $890$ & $3.93\pm2.03$ & $2.39\pm0.15$ & $29.6$ & $2.46$\\%246876040
K2-x22 b & $910$ & $7.64\pm4.5$ & $2.99\pm0.19$ & $16.4$ & $1.70$\\%246891819
K2-X22 c & $750$ & $11.81\pm7.02$ & $3.82\pm0.24$ & $19.8$ & $1.83$\\%246891819
K2-X16 b & $1990$ & $3.4\pm1.94$ & $2.56\pm0.16$ & $18.4$ & $2.31$\\%246953392
K2-X16 c & $590$ & $10.0\pm6.01$ & $2.23\pm0.14$ & $14.6$ & $0.69$\\%246953392
k2-x39 b & $1210$ & $6.74\pm4.06$ & $2.95\pm0.18$ & $28.4$ & $3.06$\\%247383003
k2-x40 b & $1240$ & $6.08\pm3.59$ & $2.17\pm0.03$ & $7.7$ & $0.68$\\%248463350
k2-x40 c & $870$ & $23.41\pm13.1$ & $5.85\pm0.09$ & $14.5$ & $1.64$\\%248463350
K2-X14 b & $2780$ & $32.28\pm22.16$ & $26.62\pm0.69$ & $51.7$ & $16.63$\\%248472140
k2-x48 b & $570$ & $1.65\pm0.8$ & $1.29\pm0.01$ & $4.0$ & $0.97$\\%248518307
K2-X24 b & $660$ & $5.83\pm3.73$ & $2.22\pm0.14$ & $15.3$ & $1.07$\\%248527514
K2-XX5 b & $870$ & $7.8\pm4.74$ & $2.0\pm0.13$ & $7.4$ & $0.52$\\%248621597
k2-x41 b & $580$ & $24.91\pm16.38$ & $5.8\pm0.36$ & $33.0$ & $2.16$\\%248758353
K2-X12 b & $450$ & $7.33\pm4.06$ & $2.95\pm0.01$ & $19.9$ & $0.76$\\%248861279
K2-X15 b & $980$ & $18.63\pm10.87$ & $7.72\pm0.48$ & $59.5$ & $9.65$\\%248874928
k2-x42 b & $720$ & $20.04\pm12.4$ & $5.27\pm0.32$ & $89.8$ & $7.82$\\%249223471
k2-x13 c & $1110$ & $2.11\pm1.14$ & $0.86\pm0.05$ & $1.8$ & $0.68$\\%249403651
k2-x13 b & $900$ & $2.49\pm1.4$ & $0.83\pm0.05$ & $1.5$ & $0.49$\\%249403651
K2-XX6 b & $610$ & $3.89\pm1.99$ & $1.04\pm0.07$ & $12.4$ & $0.44$\\%249816490
K2-XX7 b & $1800$ & $6.74\pm4.06$ & $3.77\pm0.23$ & $17.7$ & $2.21$\\%249924395

==> Table5_olderVersion.tex <==
\begin{longtable}[c]{llllll}
 \caption{Estimated values and metrics for the newly validated planets.\label{tab:estimated}}\\

 \hline
 Planet & $T_{\rm{eq}}$ [K] & $M_p$ [\mearth] & $K$ [m/s] & TSM & ESM\\ 
 \hline
 \endfirsthead

 \hline
 \multicolumn{6}{c}{Table \ref{tab:estimated} \emph{(continued)}}\\
 \hline
 Planet & $T_{\rm{eq}}$ [K] & $M_p$ [\mearth] & $K$ [m/s] & TSM & ESM\\ 
 \hline
 \endhead

 \hline
 \endfoot

 \hline\hline
 \endlastfoot
\epiczerooneonesixbalias & 710 & 8.8 & 2.2 & 21.8 & 1.3\\% EPIC204750116.01
\epicsixsixfourbalias & 770 & 6.2 & 1.8 & 18.6 & 1.1\\% EPIC205111664.01
\epicnineeightonebalias & 450 & 6.4 & 1.8 & 14.9 & 0.4\\% EPIC206055981.01
\epicsixeighttwobalias & 800 & 2.3 & 1.1 & 1.7 & 0.6\\% EPIC206135682.01
\epicsixeighttwocalias & 650 & 2.4 & 0.9 & 1.4 & 0.3\\% EPIC206135682.02
\epicsixeighttwodalias & 500 & 4.5 & 1.3 & 11.4 & 0.3\\% EPIC206135682.03
\epicninefivesevenbalias & 1080 & 2.3 & 1.0 & 2.2 & 0.8\\% EPIC206146957.01
\epictwoeightsixcalias & 570 & 5.0 & 1.4 & 8.0 & 0.3\\% EPIC206317286.01
\epicthreefiveninebalias & 1000 & 0.0 & 0.0 & inf & 38.2\\% EPIC211399359.01
\epicninenineninebalias & 870 & 9.0 & 3.0 & 12.9 & 1.0\\% EPIC211490999.01
\epiczerofivefourbalias & 1130 & 4.9 & 1.3 & 14.6 & 1.0\\% EPIC211539054.01
\epicthreeoneeightbalias & 1000 & 5.7 & 1.4 & 4.4 & 0.3\\% EPIC212006318.01
\epiconeoneeightbalias & 530 & 3.5 & 1.1 & 8.7 & 0.3\\% EPIC212530118.01
\epiceighttwoeightbalias & 1130 & 8.6 & 4.6 & 12.1 & 1.6\\% EPIC212575828.01
\epiczerosixninebalias & 680 & 5.4 & 1.9 & 17.3 & 1.0\\% EPIC214173069.01
\epicfivefourfivebalias & 1110 & 7.9 & 2.4 & 19.6 & 1.8\\% EPIC214419545.01
\epiceightthreeninecalias & 530 & 4.7 & 1.4 & 16.0 & 0.6\\% EPIC217192839.01
\epiceightthreeninebalias & 670 & 1.3 & 0.5 & 1.8 & 0.3\\% EPIC217192839.02
\epiceightthreeninedalias & 440 & 3.5 & 0.9 & 10.8 & 0.2\\% EPIC217192839.03
\epiceightninefivebalias & 610 & 4.9 & 1.2 & 10.7 & 0.4\\% EPIC217977895.01
\epicsixzerotwobalias & 1270 & 3.1 & 1.5 & 19.6 & 1.7\\% EPIC218668602.01
\epictwoseventwofalias & 370 & 5.6 & 3.1 & 28.7 & 0.5\\% EPIC220221272.01
\epictwoseventwoealias & 470 & 2.5 & 1.8 & 3.0 & 0.6\\% EPIC220221272.02
\epictwoseventwocalias & 550 & 1.8 & 1.5 & 3.0 & 0.7\\% EPIC220221272.03
\epictwoseventwoealias & 420 & 2.4 & 1.5 & 2.5 & 0.3\\% EPIC220221272.04
\epictwoseventwobalias & 680 & 1.3 & 1.3 & 4.0 & 1.1\\% EPIC220221272.05
\epicfoursevensevenbalias & 1100 & 3.0 & 1.5 & 8.0 & 0.7\\% EPIC220459477.01
\epiceightsevenfourbalias & 1010 & 6.0 & 2.1 & 12.0 & 0.9\\% EPIC220510874.01
\epictwothreethreebalias & 340 & 42.2 & 12.8 & 24.8 & 0.8\\% EPIC220696233.01
\epicfourfivefivebalias & 970 & 13.0 & 5.0 & 30.7 & 3.4\\% EPIC245943455.01
\epiczerofoureightbalias & 1050 & 5.4 & 2.0 & 17.2 & 1.2\\% EPIC245991048.01
\epiczerofoureightcalias & 780 & 4.8 & 1.3 & 11.7 & 0.6\\% EPIC245991048.02
\epicninesevensevenbalias & 1310 & 19.6 & 9.8 & 31.4 & 5.7\\% EPIC245995977.01
\epicthreeonefourbalias & 900 & 2.5 & 1.1 & 3.3 & 1.1\\% EPIC246074314.01
\epicthreenineeightbalias & 840 & 4.1 & 1.2 & 7.0 & 0.4\\% EPIC246084398.01
\epiczerofourninebalias & 950 & 6.1 & 2.0 & 16.0 & 1.2\\% EPIC246429049.01
\epicfiveeightzerobalias & 1420 & 10.4 & 5.2 & 71.4 & 9.9\\ % EPIC210797580.01 campaign 13
\epiczerofourzerobalias & 890 & 3.5 & 2.1 & 33.1 & 2.5\\% EPIC246876040.01
\epiceightoneninebalias & 910 & 7.3 & 2.8 & 17.3 & 1.7\\% EPIC246891819.01
\epiceightoneninecalias & 750 & 11.4 & 3.7 & 20.6 & 1.9\\% EPIC246891819.02
\epicthreeninetwobalias & 1990 & 3.1 & 2.3 & 20.0 & 2.3\\% EPIC246953392.01
\epicthreeninetwocalias & 590 & 9.9 & 2.2 & 14.7 & 0.7\\% EPIC246953392.02
%EPIC247164043.01 & 1410 & 5.8 & 2.2 & 44.8 & 3.8\\
\epiczerozerothreebalias & 1210 & 6.4 & 2.8 & 29.8 & 3.0\\% EPIC247383003.01
\epicthreefivezerobalias & 1240 & 5.8 & 2.1 & 8.1 & 0.7\\% EPIC248463350.01
\epicthreefivezerocalias & 870 & 22.8 & 5.7 & 14.8 & 1.6\\% EPIC248463350.02
\epiconefourzerobalias & 2780 & 30.5 & 25.1 & 54.7 & 16.6\\% EPIC248472140.01
\epicthreezerosevenbalias & 570 & 1.7 & 1.3 & 3.9 & 1.0\\% EPIC248518307.01
\epicfiveonefourbalias & 660 & 5.7 & 2.2 & 15.6 & 1.1\\% EPIC248527514.01
\epicfiveninesevenbalias & 870 & 7.6 & 2.0 & 7.5 & 0.5\\% EPIC248621597.01
\epicthreefivethreebalias & 580 & 24.6 & 5.7 & 33.2 & 2.1\\% EPIC248758353.01
\epictwosevenninebalias & 450 & 6.9 & 2.8 & 20.9 & 0.8\\% EPIC248861279.01
\epicninetwoeightbalias & 980 & 18.9 & 7.8 & 58.5 & 9.6\\% EPIC248874928.01
\epicfoursevenonebalias & 720 & 19.2 & 5.0 & 93.7 & 7.8\\% EPIC249223471.01
\epicsixfiveonebalias & 1110 & 2.2 & 0.9 & 1.7 & 0.7\\% EPIC249403651.01
\epicsixfiveonecalias & 900 & 2.4 & 0.8 & 1.5 & 0.5\\% EPIC249403651.02
\epicfourninezerobalias & 610 & 3.5 & 0.9 & 14.1 & 0.4\\% EPIC249816490.01
\epicthreeninefivebalias & 1800 & 6.7 & 3.8 & 17.8 & 2.2\\% EPIC249924395.01
\epictwooneonesixbalias & 1210 & 3.2 & 1.5 & 11.1 & 0.7\\% EPIC211732116.01
\epictwooneonesixcalias & 790 & 5.5 & 1.7 & 11.1 & 0.6\\% EPIC211732116.02
\epicthreeeightthreebalias & 1240 & 3.7 & 1.4 & 23.1 & 1.6\\% EPIC212222383.01
K2-X10 b & $710$ & $9.02\pm5.54$ & $2.29\pm0.14$ & $21.3$ & $1.26$\\
K2-X26 b & $770$ & $6.21\pm3.77$ & $1.79\pm0.11$ & $18.6$ & $1.14$\\
K2-X44 b & $450$ & $6.74\pm4.02$ & $1.89\pm0.12$ & $14.0$ & $0.41$\\
K2-X18 b & $800$ & $2.34\pm1.31$ & $1.06\pm0.07$ & $1.7$ & $0.58$\\
K2-X18 d & $650$ & $2.49\pm1.36$ & $0.91\pm0.06$ & $1.4$ & $0.35$\\
K2-X18 c & $500$ & $4.84\pm2.77$ & $1.38\pm0.09$ & $10.4$ & $0.31$\\
K2-X45 b & $1080$ & $2.2\pm1.32$ & $0.96\pm0.06$ & $2.3$ & $0.82$\\
EPIC 206317286 c & $570$ & $5.26\pm2.82$ & $1.46\pm0.09$ & $7.7$ & $0.32$\\
K2-XX4 b & $1420$ & $10.42\pm6.21$ & $5.23\pm0.32$ & $71.1$ & $9.92$\\
K2-XX1 b & $1000$ & $1610.58\pm7138.27$ & $723.7\pm46.46$ & $7.4$ & $37.84$\\
K2-X27 b & $870$ & $8.83\pm5.21$ & $2.94\pm0.05$ & $13.1$ & $1.01$\\
K2-X46 b & $1130$ & $5.26\pm3.2$ & $1.37\pm0.08$ & $13.6$ & $1.02$\\
K2-X23 b & $1210$ & $3.55\pm1.81$ & $1.69\pm0.02$ & $9.9$ & $0.75$\\
K2-X23 c & $790$ & $5.59\pm3.3$ & $1.73\pm0.03$ & $11.0$ & $0.58$\\
K2-X28 b & $1000$ & $5.71\pm3.59$ & $1.39\pm0.09$ & $4.4$ & $0.31$\\
k2-x47 b & $1240$ & $4.18\pm2.19$ & $1.59\pm0.1$ & $20.2$ & $1.61$\\
K2-X30 b & $530$ & $4.01\pm2.22$ & $1.25\pm0.08$ & $7.6$ & $0.31$\\
K2-X25 b & $1130$ & $8.3\pm5.41$ & $4.4\pm0.28$ & $12.6$ & $1.55$\\
K2-X31 b & $680$ & $5.48\pm3.65$ & $1.88\pm0.12$ & $16.9$ & $1.03$\\
K2-X32 b & $1110$ & $7.64\pm4.64$ & $2.32\pm0.14$ & $20.2$ & $1.79$\\
K2-X11 b & $670$ & $1.26\pm0.85$ & $0.49\pm0.03$ & $1.8$ & $0.34$\\
K2-X11 d & $530$ & $4.94\pm2.91$ & $1.51\pm0.1$ & $15.2$ & $0.57$\\
K2-X11 c & $440$ & $3.85\pm2.22$ & $0.99\pm0.06$ & $9.7$ & $0.20$\\
K2-XX9 b & $610$ & $5.26\pm3.07$ & $1.27\pm0.08$ & $10.0$ & $0.37$\\
K2-X33 b & $1270$ & $3.33\pm1.85$ & $1.66\pm0.1$ & $18.0$ & $1.70$\\
K2-X21 f & $600$ & $1.26\pm0.87$ & $1.54\pm0.01$ & $6.5$ & $1.44$\\
K2-X21 d & $480$ & $1.79\pm0.95$ & $1.77\pm0.01$ & $4.9$ & $0.83$\\
K2-X21 c & $410$ & $2.6\pm1.48$ & $2.2\pm0.01$ & $4.6$ & $0.60$\\
K2-X21 e & $370$ & $2.49\pm1.53$ & $1.87\pm0.01$ & $3.9$ & $0.35$\\
K2-X21 b & $330$ & $5.71\pm3.23$ & $3.82\pm0.02$ & $45.6$ & $0.54$\\
K2-X19 b & $1100$ & $3.2\pm1.68$ & $1.61\pm0.1$ & $7.5$ & $0.66$\\
k2-x34 b & $1010$ & $6.21\pm3.77$ & $2.16\pm0.03$ & $11.5$ & $0.87$\\
K2-X20 b & $340$ & $42.72\pm33.12$ & $12.97\pm0.19$ & $24.6$ & $0.83$\\
K2-XX2 b & $970$ & $13.37\pm8.36$ & $5.18\pm0.33$ & $29.7$ & $3.33$\\
K2-X17 c & $1050$ & $5.83\pm3.37$ & $2.11\pm0.13$ & $15.9$ & $1.24$\\
K2-X17 b & $780$ & $5.15\pm3.01$ & $1.39\pm0.09$ & $10.9$ & $0.55$\\
k2-x37 b & $1310$ & $19.83\pm11.81$ & $9.96\pm0.62$ & $31.0$ & $5.63$\\
K2-XX8 b & $900$ & $2.44\pm1.64$ & $1.13\pm0.07$ & $3.3$ & $1.06$\\
K2-XX3 b & $840$ & $4.45\pm2.49$ & $1.28\pm0.08$ & $6.4$ & $0.36$\\
k2-x35 b & $950$ & $6.21\pm3.93$ & $1.98\pm0.12$ & $15.9$ & $1.16$\\
k2-x36 b & $890$ & $4.01\pm2.24$ & $2.44\pm0.15$ & $29.0$ & $2.46$\\
K2-x22 b & $910$ & $7.64\pm4.41$ & $2.99\pm0.19$ & $16.4$ & $1.70$\\
K2-X22 c & $750$ & $11.81\pm7.67$ & $3.82\pm0.24$ & $19.8$ & $1.83$\\
K2-X16 b & $1990$ & $3.47\pm1.73$ & $2.61\pm0.16$ & $18.0$ & $2.31$\\
K2-X16 c & $590$ & $9.8\pm6.21$ & $2.19\pm0.14$ & $14.9$ & $0.69$\\
k2-x39 b & $1210$ & $6.6\pm3.74$ & $2.88\pm0.18$ & $29.0$ & $3.06$\\
k2-x40 b & $1240$ & $6.08\pm3.51$ & $2.17\pm0.03$ & $7.7$ & $0.68$\\
k2-x40 c & $870$ & $22.93\pm14.21$ & $5.73\pm0.09$ & $14.8$ & $1.64$\\
K2-X14 b & $2780$ & $30.02\pm21.54$ & $24.76\pm0.65$ & $55.6$ & $16.63$\\
k2-x48 b & $570$ & $1.65\pm0.83$ & $1.29\pm0.01$ & $4.0$ & $0.97$\\
K2-X24 b & $660$ & $5.71\pm3.55$ & $2.17\pm0.14$ & $15.7$ & $1.07$\\
K2-XX5 b & $870$ & $7.96\pm4.69$ & $2.05\pm0.13$ & $7.2$ & $0.52$\\
k2-x41 b & $580$ & $23.9\pm15.58$ & $5.57\pm0.34$ & $34.4$ & $2.16$\\
K2-X12 b & $450$ & $7.18\pm4.27$ & $2.89\pm0.01$ & $20.3$ & $0.76$\\
K2-X15 b & $980$ & $19.02\pm11.34$ & $7.88\pm0.49$ & $58.3$ & $9.65$\\
k2-x42 b & $720$ & $19.42\pm11.81$ & $5.11\pm0.31$ & $92.7$ & $7.82$\\
k2-x13 c & $1110$ & $2.11\pm1.11$ & $0.86\pm0.05$ & $1.8$ & $0.68$\\
k2-x13 b & $900$ & $2.49\pm1.34$ & $0.83\pm0.05$ & $1.5$ & $0.49$\\
K2-XX6 b & $610$ & $4.1\pm2.17$ & $1.09\pm0.07$ & $11.8$ & $0.44$\\
K2-XX7 b & $1800$ & $6.88\pm3.94$ & $3.85\pm0.23$ & $17.3$ & $2.21$\\
\end{longtable}
